Bag of Attributes for Video Event Retrieval

In this paper, we present the Bag-of-Attributes (BoA) model for video representation aiming at video event retrieval. The BoA model is based on a semantic feature space for representing videos, resulting in high-level video feature vectors. For creating a semantic space, i.e., the attribute space, we can train a classifier using a labeled image dataset, obtaining a classification model that can be understood as a high-level codebook. This model is used to map low-level frame vectors into high-level vectors (e.g., classifier probability scores). Then, we apply pooling operations to the frame vectors to create the final bag of attributes for the video. In the BoA representation, each dimension corresponds to one category (or attribute) of the semantic space. Other interesting properties are: compactness, flexibility regarding the classifier, and ability to encode multiple semantic concepts in a single video representation. Our experiments considered the semantic space created by state-of-the-art convolutional neural networks pre-trained on 1000 object categories of ImageNet. Such deep neural networks were used to classify each video frame and then different coding strategies were used to encode the probability distribution from the softmax layer into a frame vector. Next, different pooling strategies were used to combine frame vectors in the BoA representation for a video. Results using BoA were comparable or superior to the baselines in the task of video event retrieval using the EVVE dataset, with the advantage of providing a much more compact representation.

==> Makefile <==
### Makefile
### $Id: Makefile,v 1.11 2006/06/26 04:51:29 jurandy Exp $

CP = cp
MV = mv
RM = rm

EGREP = egrep

LATEX = latex
BIBTEX = bibtex
DVIPS = dvips
PS2PDF = ps2pdf
PDFLATEX = pdflatex

BIBFLAGS = -min-crossrefs=32768
DVIFLAGS = -t letter -Ppdf -Pbuiltin35 -G0
PSFLAGS = -sPAPERSIZE=letter -dCompatibilityLevel=1.2 -dEmbedAllFonts=true -dPDFSETTINGS=/prepress
PDFFLAGS = -shell-escape


RERUN = "Rerun to get (cross-references|the bars) right"
RERUNBIB = "No file.*\.bbl"

SRC = $(shell egrep -l '^[^%]*\\begin\{document\}' *.tex)

all: install clean

install: pdftex

uninstall:
	$(RM) -f $(SRC:%.tex=%.dvi) $(SRC:%.tex=%.ps) $(SRC:%.tex=%.pdf)

%.dvi:	%.tex
	$(LATEX) $<
	$(EGREP) -c $(RERUNBIB) $*.log && $(BIBTEX) $(BIBFLAGS) $* ; true
	while ( $(LATEX) $< ; $(EGREP) -c $(RERUN) $*.log ) do true ; done
	$(EGREP) -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:	%.dvi
	$(DVIPS) $(DVIFLAGS) $< -o $@

%.dpp:	%.ps
	$(PS2PDF)  $(PSFLAGS) $<

%.pdf:	%.tex
	$(PDFLATEX) $(PDFFLAGS) $<
	$(EGREP) -c $(RERUNBIB) $*.log && $(BIBTEX) $(BIBFLAGS) $* ; true
	while ( $(PDFLATEX) $(PDFFLAGS) $< ; $(EGREP) -c $(RERUN) $*.log ) do true ; done
	$(EGREP) -i "(Reference|Citation).*undefined" $*.log ; true

%.pic:	%.dpp
	$(MV) $*.pdf $*-pics.pdf

%.p4f:	%.pic %.pdf
	$(RM) -f $*.dvi $*.ps $*-pics.pdf

dvi:	$(SRC:%.tex=%.dvi)
ps:		$(SRC:%.tex=%.ps)
dvips:	$(SRC:%.tex=%.dpp)
pdftex:	$(SRC:%.tex=%.pdf)
ps4pdf:	$(SRC:%.tex=%.p4f)

clean:
	$(RM) -f *-pics.* core *.core *.log *.aux *.toc *.lo[fpta] \
	*.blg *.brf *.ind *.ilg *.idx *.glo *.gls *.nav *.snm *.pfg *.out

### Makefile ends here.


